Dynamic Proxy-Mixing: Transferring Replay Controllers from Small to Large Models for Continual Instruction Tuning

Continual instruction tuning updates a language model through a sequence of new domains, yet each update can progressively erode previously learned capabilities and alignment behavior. Replay is the standard mitigation, but fixed replay ratios are inherently limited because the optimal mixture varies with the current domain, the training stage, and the evolving vulnerability of prior behaviors. We propose PROX-YMIX, a framework that learns a dynamic replay controller on a small proxy model and transfers the frozen controller to a larger target. The controller never observes future tasks and constructs its state from normalized validation losses and their temporal dynamics, producing a masked mixture over the current task and accessible replay buffers. Our core empirical hypothesis is forgetting mirroring: task vulnerability rankings remain largely consistent across model scales even when absolute loss magnitudes differ. We validate this assumption empirically before transferring controllers across scales. On LLaMA-3-8B across five continual instruction tuning sequences, PROXYMIX improves average accuracy by 3.4 points, reduces final forgetting by 3.5 points, and raises safety score by 5.8 points over the strongest non-oracle baseline, at roughly 50x lower policy learning cost than Oracle Target RL. The framework is leakage free and architecture independent at the interface level, and we also identify settings where the proxy assumption breaks down, highlighting limitations for robust deployment.

==> updates.tex <==
Update Figure 5 and Figure 6 data

Regenerate Appendix Figure 5 and Figure 6 from the updated Table 11 values:

S1: AA 70.1, FGT 6.3,  NTA 71.9, BWT -3.0, SS 89.7
S2: AA 63.4, FGT 10.4, NTA 69.1, BWT -8.4, SS 81.0
S3: AA 67.9, FGT 10.3, NTA 70.7, BWT -4.6, SS 85.3
S4: AA 62.3, FGT 9.8,  NTA 68.0, BWT -7.3, SS 84.5
S5: AA 70.8, FGT 6.2,  NTA 72.3, BWT -2.2, SS 88.5

Figure 6 should use only:

S1: 70.1
S2: 63.4
S3: 67.9
S4: 62.3
S5: 70.8



Yes, **you can keep Figure 13**, but **not in its current form**. Right now it contradicts your method section and looks like a leftover figure from a different controller design.

Figure 13’s caption says the state is built from “validation losses from previous tasks,” normalized, trended, and masked before being fed to the controller.  But your actual method says the controller state includes **visible tasks** (A_t={1,\ldots,k(t)}), including the current task, uses normalized losses and trend terms for all visible tasks, includes (e_{k(t)}) and progress (p_t), and outputs replay-mixture logits through a masked softmax. 

## What must change in Figure 12

### 1. Remove “previous tasks only”

Current Figure 13 says “Validation Losses (Per Previous Task).” That is wrong.

Change to:

```text
Validation losses over visible tasks
i ∈ A_t = {1, ..., k(t)}
```

The current task must be included because Eq. 4 includes visible tasks and Eq. 6 uses the current-task trend term.

---

### 2. Replace “Min–Max Normalization”

Current Figure 13 shows:

```text
L_i^norm = (L_i^val - L_min) / (L_max - L_min)
```

But your method uses running mean/variance normalization in Eq. 3, not min–max normalization. 

Change the box to:

```latex
\tilde{\ell}^{(t)}_i =
\frac{\ell^{(t)}_i - \mu^{(t)}_i}
{\sqrt{v^{(t)}_i+\epsilon}}
```

Label it:

```text
Running z-normalization
```

---

### 3. Replace the trend formula

Current Figure 13 uses a moving-window difference formula. Your method defines trend as:

```latex
\Delta \tilde{\ell}^{(t)}_i =
\tilde{\ell}^{(t)}_i - \tilde{\ell}^{(t-\delta)}_i
```

Use exactly that. Label it:

```text
Temporal loss trend over controller interval δ
```

---

### 4. Fix the masking rule

Current Figure 13 says:

```text
M_i = 0, i = k
M_i = 1, otherwise
```

That masks the current task, which is wrong. Your masked softmax allows the current task and past tasks, and masks only future tasks: (m_i^{(t)}=\mathbb{1}[i\le k(t)]). 

Change to:

```latex
m_i^{(t)} = \mathbb{1}[i \le k(t)]
```

Label it:

```text
Mask future tasks only
```

And add:

```text
Future tasks are zero-filled in the state and excluded from the action distribution.
```

---

### 5. Fix the state vector

Current Figure 13 shows something like:

```text
s_t = [τ_1 M_1, τ_2 M_2, ..., τ_k M_k]
```

But Eq. 4 defines the state as normalized losses, trends, current-task one-hot, and within-task progress. 

Replace the state-vector box with:

```latex
s_t =
[
\bar{\ell}^{(t)}_1,\ldots,\bar{\ell}^{(t)}_T,
\Delta\bar{\ell}^{(t)}_1,\ldots,\Delta\bar{\ell}^{(t)}_T,
e_{k(t)}, p_t
]
```

Add a small note:

```text
Masked entries for i > k(t) are zero-filled.
```

---

### 6. Remove the controller outputs “LoRA rank / LoRA scaling / proximal strength”

This is the most serious issue. Your PROXYMIX controller does **not** output LoRA rank, LoRA scaling, or proximal strength. It outputs replay-mixture logits (a_t \in \mathbb{R}^T), then a masked softmax gives mixture weights (w_i^{(t)}). 

Replace the output box with:

```text
Output:
replay logits a_t ∈ R^T
```

Then add:

```latex
w_i^{(t)} =
\frac{m_i^{(t)} \exp(a_i^{(t)})}
{\sum_{r=1}^{T} m_r^{(t)} \exp(a_r^{(t)})}
```

Label:

```text
Masked replay mixture over current and replay buffers
```

---

## Replace the Figure 13 caption

Use this caption:

```latex
\caption{Masked state construction for PROXYMIX. At each controller decision step, validation losses are computed for the current visible task set $A_t=\{1,\ldots,k(t)\}$. Losses are normalized with running per-task statistics, temporal trends are computed over the controller interval $\delta$, and future-task entries are zero-filled. The resulting fixed-dimensional state concatenates normalized losses, trend features, a one-hot current-task index, and within-task progress before being passed to the PPO controller. The controller outputs replay logits, which are converted into a masked mixture over the current task and accessible replay buffers.}
```

## Also change the Appendix K intro

Current Appendix K says supplementary figures illustrate “controller design, per-sequence robustness, and proxy-scaling behavior.” That is okay, but Figure 13 needs to be explicitly tied to Eq. 4–5.

Add this sentence before Figure 13:

```latex
Figure~13 expands the masked state construction in Eq.~4 and the future-task masking used in Eq.~5.
```

